Unsupervised Social Bot Detection via Structural Information Theory

Research on social bot detection plays a crucial role in maintaining the order and reliability of information dissemination while increasing trust in social interactions. The current mainstream social bot detection models rely on black-box neural network technology, e.g., Graph Neural Network, Transformer, etc., which lacks interpretability. In this work, we present UnDBot, a novel unsupervised, interpretable, yet effective and practical framework for detecting social bots. This framework is built upon structural information theory. We begin by designing three social relationship metrics that capture various aspects of social bot behaviors: Posting Type Distribution, Posting Influence, and Follow-to-follower Ratio. Three new relationships are utilized to construct a new, unified, and weighted social multi-relational graph, aiming to model the relevance of social user behaviors and discover long-distance correlations between users. Second, we introduce a novel method for optimizing heterogeneous structural entropy. This method involves the personalized aggregation of edge information from the social multi-relational graph to generate a two-dimensional encoding tree. The heterogeneous structural entropy facilitates decoding of the substantial structure of the social bots network and enables hierarchical clustering of social bots. Thirdly, a new community labeling method is presented to distinguish social bot communities by computing the user's stationary distribution, measuring user contributions to network structure, and counting the intensity of user aggregation within the community. Compared with ten representative social bot detection approaches, comprehensive experiments demonstrate the advantages of effectiveness and interpretability of UnDBot on four real social network datasets.

==> background.tex <==
\section{Background and Overview}
\label{sec:background} 


\subsection{Problem Definition}

In this section, we will first define multi-relational graphs and introduce Structural Entropy. Following this, we will provide a summary of the problems and challenges that must be addressed. Additionally, a comprehensive list of the primary symbols used throughout this paper can be found in Table 1.


\begin{table}[b]
\caption{Notations.} 
\small 
\centering
\begin{tabular}{r|l} 
\hline\hline
\textbf{Symbol} & \textbf{Definition} \\
\hline
$\mathcal{G}; \mathcal{G}^r$ & Homogeneous Graph; Multi-relational Graph\\
\hline
$\mathcal{V};\mathcal{E}; \mathcal{E}_r$ & Vertices set; Edge set of Homogeneous Graph; Edge set under relationship $r$ \\
\hline
$r; R$ & Relation; Total number of relations\\
\hline
$v; N$ & Vertex in graph; Total number of vertices \\
\hline
$e_{i,j}^r$ & edge between vertex $i$ and vertex $j$ under relationship $r$\\
\hline
$\mathcal{T}; \lambda$ & Encoding tree; The root node of the encoding tree \\
\hline
$ \alpha;T_\alpha$ & The node on encoding tree; Label of node $\alpha$ \\
\hline
$\alpha_i; \alpha^-$ & Child node of node $\alpha$; Parent node of node\\
\hline
$d_i; g_\alpha$ & Degree of vertex $i$; Number of cutting edges of node $\alpha$ \\
\hline
$vol(\mathcal{G}); vol(\alpha)$ & Volume of Graph $\mathcal{G}$; Volume of node $\alpha$\\
\hline
$H^\mathcal{T}(\mathcal{G})$ & The structural information under encoding tree $\mathcal{T}$\\
\hline
$H_k(\mathcal{G})$ & The K-dimensional structure entropy\\
\hline
$H(\mathcal{G}^r;\alpha)$ & Entropy of node $\alpha$ on an encoding tree\\
\hline
$Pt; Inf; ff$  & Distribution of posting types; Influence of posting; Following-followers ratio\\
\hline
$d_{i,j}$ & Manhattan distance between posting type distribution between user $i$ and user $j$\\
\hline
$\Delta_{i,j} $ & Deviation ratio of influence between user $i$ and user $j$\\
\hline
$\xi_T$ &  Threshold of the similarity for posting type distribution\\
\hline
$\xi_I$ &  Threshold of the similarity for posting influence\\
\hline
$\xi_F$ &  Threshold of the similarity for Following-followers ratio\\
\hline
$Mg(\mathcal{T};\alpha,\beta)$ & Merging operator between node $\alpha$ and node $\beta$\\
\hline
$\mathcal{T}_{mg}$ & Encoding tree after Merging operator\\
\hline
$\Delta_{\mathcal{G}^r}^{Mg}(\mathcal{T};\alpha,\beta)$ & Difference of Structural entropy after merging node $\alpha$ and $\beta$\\
\hline
$A$ & A three-dimensional tensor of multi-relational graph $\mathcal{G}^r$\\
\hline
$O$ & Tensor of transition probabilities to reach different vertices\\
\hline
$R$ & Tensor of transition probabilities through different edges\\
\hline
$o_{i,j,k}$ &  the possibility of reaching vertex $v_j$, from vertex $v_i$ through $k$-th edge\\
\hline
$r_{i,j,k}$ &  the possibility of going through $k$-th edge, from vertex $v_i$ to vertex $v_j$\\
\hline
$X; Y$ &  stationary distribution of users; stationary distribution of edges\\
\hline
$E(\alpha)$ & Evaluation score of the community represented by node $\alpha$\\
\hline
$\xi_C$ & Threshold of evaluation index for communities\\
\hline\hline
\end{tabular}
\label{tab:notation}
\end{table} 


\begin{defn}
\label{def: Multi-Relational Graph}
\textbf{Multi-Relational Graph.}

The multi-relational graph denoted as $\mathcal{G}^r=\{\mathcal{V},{\mathcal{E}_{r}}|_{r=1}^{R}\}$, is defined in terms of $\mathcal{V}$ and $\mathcal{E}_{r}$, where $\mathcal{V}$ representing the set of vertices $\{v_{1}, \dots, v_{N}\}$, and $N$ denotes the total number of vertices in the set.
$\mathcal{E}_{r}$ represents the set of edges $e_{i, j}^{r} = (v_{i}, v_{j})\in \mathcal{E}_{r}$ defined between vertices under relation $r$, where $R$ is the number of different kinds of relationships. 
The multi-relational graph takes the elements to be classified as vertices and several important relationships between different vertices as edges to model the real network.
However, unlike simple homogeneous graphs, multi-relational graphs contain richer structural and semantic information by taking into account the heterogeneity between edges.
It is different from the multi-vertex and multi-relationship heterogeneous information network(HIN), as the multi-relational graph has only one vertex type but multiple edge relations between the vertices. 
This approach intuitively and flexibly reflects the connection between elements to be classified, and there is no need to manually define meta-paths between different vertices to specify semantic connections between entities, as in the case of a HIN.

The following uses the social bot detection to be studied in this paper to describe the application of the multi-relational graph in detail and compare it with the modeling methods of the homogeneous graph and the heterogeneous information network.
Social bots, also known as machine accounts, refer to non-human accounts on social platforms such as Twitter, Facebook, Weibo, etc., which are a major hazard to social trust and the orderly dissemination of information.
We regard the accounts of social platforms as vertices, and the commonality of social behavior between social accounts as different types of edges to construct a multi-relational graph, thereby transforming social bot detection into a binary classification problem of community detection.
As shown in Figure xx, a social user behavior network is modeled with a multi-relational graph, including human accounts, machine accounts, and different types of connections between users. 
The connections we selected are closely related to social bots, including the same post type distribution, the same post influence, and the same follower ratio.
Figure xx shows a social network model with a homogeneous graph, whose edges have a single meaning and cannot well reflect multiple interactions and connections between social accounts.
Figure xx shows a social network model with a heterogeneous graph, whose vertex types include users, tweets, comments, etc. 
The internal connection structure is complex, and the artificially defined meta path pays more attention to certain structured connections, such as "user-tweet-user", etc. 
\end{defn}


\begin{defn}
\label{def: Structural Entropy}
\textbf{Structural Entropy.}
Structural information theory~\cite{li2016structural} was originally proposed in 2016 for measuring the structural information contained within a graph. Specifically, this theory aims to calculate the structural entropy of the homogeneous graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, which reflects its uncertainty when undergoing hierarchical division. 
We introduce encoding trees and K-dimensional structural entropy below.

\textbf{Encoding tree}
An encoding tree of a graph $\mathcal{G}$ is defined as a rooted tree $\mathcal{T}$ with the following properties:
\begin{enumerate}
\item For each node $\alpha$ in the encoding tree $\mathcal{T}$, there is a subset $T_{\alpha} \in \mathcal{V}$ of vertices in the graph $\mathcal{G}$ corresponding to it.
\item For the root node $\lambda$ in the encoding tree, $T_\lambda=\mathcal{V}$.
\item The children of node $\alpha$ are denoted as $\alpha_{i}$ and sorted from left to right as $i$ increases. 
The parent node of $\alpha_{i}$ is denoted as $\alpha_{i}^-=\alpha$.
\item If node $\alpha$ has $L$ children, then the vertex subset $T_{\alpha_{i}}$ of child nodes is mutually exclusive, and $T_{\alpha}=\cup T_{\alpha_{i}}$.
\item Each leaf node $v$ in the tree, $v$ corresponds to a single vertex in the vertex set $\mathcal{V}$ in the graph $\mathcal{G}$.
\end{enumerate}
The K-dimensional encoding tree means that the height of the tree is k (the height of the root node is 0).
Intuitively, the encoding tree embodies the hierarchical community division of graph vertices, the parent node is a large community and the child nodes are small communities in the large community.

\textbf{structure entropy }
The structural information of the homogeneous graph $\mathcal{G}$ determined by the encoding tree $\mathcal{T}$ is defined as:
\begin{eqnarray} 
H^\mathcal{T}(\mathcal{G})=-\sum_{\alpha \in \mathcal{T},\alpha \neq \lambda}\frac{g_\alpha}{vol(\mathcal{G})}log\frac{vol(\alpha)}{vol(\alpha^-)}
\end{eqnarray}
Where $vol(\mathcal{G})$ is the sum of the degrees of all vertices in the graph $\mathcal{G}$. 
$vol(\alpha)$ is the volume of $T_{\alpha}$ and is the sum of the degrees of all vertices in the vertex subset $T_{\alpha}$. 
$g_{\alpha}$ is the sum of weights of all edges from vertex subset $T_{\alpha}$ to vertex subset $\mathcal{V}/ T_{\alpha}$, which can be understood as the total weight of the edges from the vertices outside the vertex subset $T_{\alpha}$ to the vertices inside the vertex $T_{\alpha}$, or the total weight of the cut edges.
$\frac{g_\alpha}{vol(\mathcal{G})}$ represents the probability that the random walk enters $T_{\alpha}$.
The structural entropy $H(\mathcal{G})$ of graph $\mathcal{G}$ is the minimum $H^{\mathcal{T}}(\mathcal{G})$. 
Let $\mathcal{T}_k$ be encoding trees whose height is not greater than K, then the K-dimensional structural entropy of $\mathcal{G}$ is defined as follows:
\begin{eqnarray} 
H_k(\mathcal{G})=min H^{\mathcal{T}_k}(\mathcal{G})
\end{eqnarray}

One-dimensional structural entropy is special there are only root nodes and leaf nodes in the encoding tree of one layer.
All the vertices in the graph $\mathcal{G}$ belong to a large community $\lambda$ under the one-dimensional encoding tree, which is unique in terms of community division, so the one-dimensional structural entropy can be directly expressed as:
\begin{eqnarray} 
H_1(\mathcal{G})=-\sum_{i=1}^{n}\frac{d_i}{vol(\mathcal{G})}log\frac{d_i}{vol(\mathcal{G})}
\end{eqnarray}
Where $d_i$ is the sum of weights of all edges connected to vertex $v_i$ in graph $\mathcal{G}$ and is called the degree of vertex $v_i$. 
One-dimensional structural entropy measures the uncertainty of graph $\mathcal{G}$ without layering.
\end{defn}



\subsection{Problem Scope and Challenges}
\label{sec:challenges}
For practical tasks, we model with multi-relational graphs to transform the social bot detection problem into an unsupervised vertex classification problem.
According to the two-dimensional structural entropy minimum algorithm, the vertices in the graph can be clustered hierarchically. 
Once the social user community is formed, the next task is to classify the community.
To achieve efficient, unsupervised, and interpretable user vertices classification, social bot detection faces the following 3 main challenges:

\textbf{How to model social user networks from the perspective of social bots? (Challenge 1)} 

The majority of the current graph modeling approaches create links between users based on their direct interactions on social networks, such as liking, commenting, retweeting, favoriting, following/being followed, and mentioning.
Although this technique can intuitively capture the interactions between social users and facilitate neighbor aggregation of the graph neural network to learn high-order user features, it has minimal impact on the detection of social bots from a network structure point of view.
Given the increasing intelligence of social bots, their interactions with actual users are becoming more commonplace.
A large quantity of bots infiltrates typical human social networks, which are hard to detect via social network structure information modeled solely by interaction relationships~\cite{ferrara2016rise}.
Hence, it is necessary to define new types of social relationships and model a social user network from the hidden behavior commonality of social bots.

\textbf{How to achieve adaptive hierarchical clustering of social users(Challenge 2)?} 

There are currently two types of clustering algorithms used in social bot detection: feature-based clustering algorithms and network structure-based community detection algorithms~\cite{chen2017people}, such as K-nearest neighbors, density clustering, maximum flow minimum cut theory, etc. 
However, these classic models have a single level of user clustering. 
The structural information theory, proposed in 2016, can decode the essential structure of social networks, and build a structural entropy encoding tree to achieve adaptive hierarchical community division of social users. 
However, the current structural entropy optimization strategy is aimed at homogeneous networks and does not consider the heterogeneity of user relationships in social network environments. 
Therefore, a structure entropy optimization strategy under multi-relational graphs is needed to achieve adaptive hierarchical clustering of social users.

\textbf{How to label social user communities and implement binary classification(Challenge 3)?}

The structural entropy of a multi-relational graph can only achieve the effect of clustering users and cannot directly separate users into two communities of social bots and humans. 
Moreover, the number of communities formed on the encoding tree depends on the structure of the multi-relational graph.
Although it is possible to observe that normal human users form some communities and social bots form other communities on the encoding tree, without sample labeling, it is not possible to determine which communities are bot communities.

